Constant Time Updates in Hierarchical Heavy Hitters

Monitoring tasks, such as anomaly and DDoS detection, require identifying frequent flow aggregates based on common IP prefixes. These are known as \emph{hierarchical heavy hitters} (HHH), where the hierarchy is determined based on the type of prefixes of interest in a given application. The per packet complexity of existing HHH algorithms is proportional to the size of the hierarchy, imposing significant overheads. In this paper, we propose a randomized constant time algorithm for HHH. We prove probabilistic precision bounds backed by an empirical evaluation. Using four real Internet packet traces, we demonstrate that our algorithm indeed obtains comparable accuracy and recall as previous works, while running up to 62 times faster. Finally, we extended Open vSwitch (OVS) with our algorithm and showed it is able to handle 13.8 million packets per second. In contrast, incorporating previous works in OVS only obtained 2.5 times lower throughput.

==> OVS_graphs/ovseval.tex <==

\section{Open vSwitch Implementation}
Next, we evaluate a prototype implementation of the proposed HHH algorithms in OVS. We first provide an overview of OVS architecture. Then, we dive into how HHH are implemented in OVS and on its performance.

\input{ovsOverview}

\subsection{Implementation Design}
We implement HHH algorithms as part of the dataplane ... 

%The first uses Skipper as a dynamic sampling technique and performs the measurement in a separate virtual machine that can be placed anywhere in the cloud.
%A second option is to perform the measurement itself inside of the data plane as an integral path of the datapath.
%This alternative yields higher throughput as data is transmitted to the measurement VNF. However, this alternative creates coupling between the measurement algorithm and the virtual switch.
%These options are illustrated in Figure~\ref{fig:dut}.

%implementation where network monitoring is an integral part of the tasks performed by the datapath. 

%That is, it provides the capability to dynamically adjust the sample interval, the sampled packets are then forwarded to a virtual machine that contains the measurement algorithm. This implementation offers more flexibility, and is in line with the NFV paradigm. The drawback of this implementation are the additional overheads that are imposed by switching traffic toward a separate VNF.  
 
%It is important to note that, while our implementation deal to DPDK-accelerated datapath, they can easily be adopted to other versions. 

%Second, we consider that the back box HH algorithm (in our case SSH) is running apart of OVS. This particular design is essential to understand and assess since decoupling network functionalities (in this case, the monitoring) is one of the main advantages and premises of NFV. 
%
%For this implementation, we basically forward packets to the black box VNF according to the adaptive update probability. Our proposed sampling implementation redefines a forwarding action as a 'branch' of the datapath. Sampled packets are actually forwarded and unsampled packets are just dropped.


%Our Skipper implementation extends the DPDK accelerated datapath capabilities, it is very local and only touch the dpif component, in Figure \ref{fig:ovs}. As packets are processed through the datapath, we retain easy access to the packet metadata.  Our proposed sampling implementation redefines a forwarding action as a 'branch' of the datapath. Sampled packets are actually forwarded and unsampled packets are dropped. Hence, our core implementation is simple and only requires few lines of code in dpif-netdev. Although our implementation is tailored to DPDK-accelerated user space datapath, its implementation on kernel versions is straightforward.



\subsection{Evaluation}
\subsubsection{Environment setup}

Our evaluation settings consist of two identical HP ProLiant servers with an Intel Xeon E3-1220v2 processor running at 3.1 Ghz with 8 GB RAM. Both servers are equipped with DPDK-enabled network interface cards (Intel 82599ES 10 Gbit/s). Each server is directly interconneced through a different physical interface. The servers run CentOS 7.2.1511 with Linux kernel 3.10.0. 

We use one server as \emph{Design Under Test (DUT)}, and the other as a traffic generator. In our \emph{DUT}, we use Open vSwitch 2.5 compiled with Intel DPDK 2.02. NIC physical ports are attached to OVS using \emph{dpdk} ports. OVS is configured so as all incoming network traffic is forwarded to another interface. In the traffic generator, we rely on the MoonGen traffic generator~\cite{MoonGen2015} tool to generate traffic at line rate. We generate UDP network traffic according to dataset Chicago16. We keep the source and destination IP prefixes as they are in the dataset and adjust the payload size in order to generate packets of 64 Bytes (reaching up to 14.88 Mpps in 10 Gbit/s NICs).

%MoonGen sends packets through one network interface and receives them on the other one after being processed by OVS.


%Scenario
%\subsubsection{Alternative Solutions}
%We evaluate the OVS performance considering the implementation of HHH algorithms.  We compare the performance of OVS without running any HHH algorithm (baseline) against our proposed solutions (RHHH and FRHHH). We compare them to Partial Ancestry implementation.

% as part of the OVS dataplane. All implementations consider the 2D Byte version. We also compare them against the case where OVS samples the packets to a third-party VNF that implements HHH algorithms. 


\begin{figure}[t]\centering
	\includegraphics[width = \columnwidth, height=5cm]{graph1.pdf}
	\caption{Measured throughput using different HHH implementations.}
	\label{fig-bw1}
\end{figure}

\begin{figure}[t]\centering
	\includegraphics[width = \columnwidth, heigInht=5cm]{graph2.pdf}
	\caption{Measured throughput of FRHHH using different filter probabilities.}
	\label{fig-bw2}
\end{figure}

\subsubsection{Results}
Figure \ref{fig-bw1} illustrates the throughput of OVS when running HHH algorithm in dataplane. For the evaluations, we consider $\epsilon = 2^10$. We compare our proposal solutions (RHHH and FRHHH) against OVS (without any HHH) and with Partial Ancestry algorithm. Observe that Partial Ancestry algorithm leads to an overhead in terms of throughput greater than 60\% in comparison to OVS baseline. In contrast, our proposal, FRHHH, leads to a negligeable throughput overhead (lower than 3\%).% , while RHHH to $~20\%$.

In Figure \ref{fig-bw2}, we illustrate the impact of different filter probabilities on the overhead of FRHHH method. Observe that as we increase the probability to update HHH, the throughput overhead increases (up to 25\%) since more packets update the HHH data structures. Observe that there is a tradeoff between the error and the achieved performance.
%
Additionally, we also compare FRHHH to the scenario which packets are sampled to a monitoring VNF. In this particular case, we assume that the VNF has an implementation of HHH. Then, OVS is required to forward a percentage of packets to that VNF. As OVS does not support natively sampling packets in the dataplane, we implement a packet uniform sampling method in the dataplane so as OVS also forwards packets to a virtual port (attached to the VNF). Observe, in Figure \ref{fig-bw2}, that considering a probability of 10\% on sampling the packets, higher penalties are obtained than doing it for 30\% of the packets in the dataplane. 


%Figure \ref{fig-bw} shows the average end-to-end throughput on the SanJose14 trace for our two designs. Similar results were obtained when running different network traces.
%As shown, measuring the data inside the data plane is efficient and reduces the throughput by only $3\%$. 
%When the measurement takes place in a dedicated VNF, Skipper increases the OVS throughput by about $25\%$.
%When the measurement is done as a part of the datapath its overheads are almost negligible and the throughput impact is less than $3\%$. The reason for that is that less traffic is routed. Alternatively, when Skipper is implemented as a VNF, the measurement reduces throughput by $13\%$, when compared to not performing measurement. Since sketches and counter based algorithms process all packets in the stream, implementing them as VNFs has higher overheads, and degrades performance by more than $30\%$. 


%We clearly observe the existence of a tradeoff between flexibility and performance between the two proposed designs. Running the monitoring HH algorithm outside OVS (in a VNF) introduces higher flexibility in the implementations of new HH strategies. In turn, compiling HH algorithm as part of the OVS datapath reduce the burden of forwarding packets to a VNF.
%




==> notationsTable2.tex <==
\begin{table}[h]
	\centering
	

	
	\begin{tabular}{|c|l|}
		
		\hline
		Symbol & Meaning \tabularnewline
		\hline
		$\mathbb{S}$ & Stream \tabularnewline
		\hline
		$N$ & Current number of packets (in all flows)  \tabularnewline
		\hline
		$H$ & Size of Hierarchy  \tabularnewline
		\hline
		$V$ & Performance parameter, $V\ge H$  \tabularnewline
		\hline
		$S^i_x$ & Variable for the i'th appearance of a prefix $x$. 
		\tabularnewline
		\hline
		$S_{x}$ & Sampled prefixes with id $x$. 
		\tabularnewline
		\hline
		$S$ &  Sampled prefixes from all ids. 
		\tabularnewline
		
		\hline
		$\mathcal U$ & Domain of fully specified items. \tabularnewline
		\hline
		$\epsilon,\epsilon_s,\epsilon_a $ & Overall, sample, algorithm's error guarantee.  \tabularnewline
		\hline
		$\delta,\delta_s , \delta_a$ &   Overall, sample, algorithm confidence. \tabularnewline
		\hline
		$\theta$ & Threshold parameter.    \tabularnewline
		\hline

		$C_{q|P}$ & Conditioned frequency of $q$ with respect to  $P$ \tabularnewline
		\hline
		$G(q|P)$ & Subset of $P$ with the closest prefixes to q.  \tabularnewline
		\hline
		$f_q$ & Frequency of prefix q \tabularnewline
		\hline
		$\widehat{f^{+}_q},\widehat{f^{-}_q}$ & Upper,lower bound for $f_q$  \tabularnewline
		\hline
	\end{tabular}
	\caption{List of Symbols}
	\label{tbl:notations}
	
\end{table}

==> xstring.tex <==
%  __________________________________________________
% |                                                  |
% |                                                  |
% |                   xstring v1.7c                  |
% |                                                  |
% |                  13 octobre 2013                 |
% |                                                  |
% |__________________________________________________|
%
% This is xtring.tex
%
% "xstring" package consists of the 7 following files:
%   xstring.tex (this file)
%   xstring.sty
%   README
%   xstring_doc_fr.tex, xstring_doc_fr.pdf (manual in french)
%   xstring_doc_en.tex, xstring_doc_en.pdf (manual in english)
%
% Christian Tellechea 2008-2013
% email : unbonpetit@gmail.com
% -------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
%     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% -------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% -------------------------------------------------------------------
\def\xstringversion     {1.7c}
\def\xstringdate        {2013/10/13}
\def\xstringfrenchdate  {13 octobre 2013}
\def\xstringenglishdate {13 october 2013}
\edef\CurrentAtCatcode  {\the\catcode`\@}
\catcode`\@=11
\newwrite\@xs@message% canal pour les messages
\newcount\integerpart
\newcount\decimalpart% compteurs utilis\'es par xstring

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\immediate\write\m@ne{Package: xstring \xstringdate\space\space v\xstringversion\space\space String manipulations}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
\fi% fin des d\'efinitions LaTeX

\long\def\@xs@ifempty#1{%
	\expandafter\ifx\expandafter\relax\detokenize{#1}\relax
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}
% Ouvre un groupe o\`u les catcodes sont \`a 12 et \`a 10 pour les espaces
% ensuite, appelle \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\@xs@MakeVerb{% lit 1 argument et le transforme en verb
	\begingroup% groupe o\`u les catcodes sont \`a 12 pour la lecture suivante
		\def\do##1{\catcode`##112\relax}%
		\dospecials% on entre dans le mode verb
		\obeyspaces% et on tient compte des espaces
		\@xs@ReadVerb% et on va lire l'argument
}

% D\'efinit \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\setverbdelim#1{% d\'efinit quel est le d\'elimiteur de verb
	\expandafter\@xs@ifempty\expandafter{\@gobble#1}%
		\relax
		{\begingroup
			\newlinechar`\^^J%
			\immediate\write\@xs@message
			{Package xstring Warning: verb delimiter is not a single token on input line \the\inputlineno^^J}%
		\endgroup
		}%
	\def\@xs@ReadVerb##1#1##2#1{% lit ##2 qui est entre les d\'elimiteurs de verb
		\endgroup% on ferme le groupe
		\@xs@afterreadverb{##2}}% on appelle l'ex\'ecution de fin
}

% Assigne l'argument entre d\'elimiteur verb dans la sc #1' +
\def\verbtocs#1{%
	\def\@xs@afterreadverb##1{\def#1{##1}}%
	\@xs@MakeVerb
}

\begingroup
	\catcode\z@3 \def\@xs@twochars{^^00}%
	\catcode\z@7 \xdef\@xs@twochars{\@xs@twochars^^00}%
\endgroup

\edef\@xs@reserved@A{\long\def\noexpand\@xs@AssignResult##1\@xs@twochars}

\@xs@reserved@A#2{\endgroup\expandafter\def\expandafter#2\expandafter{\@gobble#1}}

\def\tokenize#1#2{%
	\begingroup
		\@xs@def\@xs@reserved@A{#2}% on d\'eveloppe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\@xs@twochars#1}% met "^^@^^@#1" \`a la fin du fichier virtuel
		\endlinechar\m@ne
		\expandafter\@xs@AssignResult\scantokens\expandafter{\expandafter\relax\@xs@reserved@A}% on fait l'assignation
}%

% Macro tr\`es simple qui assigne ou affiche le r\'esultat, selon la pr\'esence
% ou non de #2 qui est l'argument optionnel venant en derni\`ere position des macros
\long\def\@xs@ReturnResult#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#2}%
		\@xs@argument@A
		{\let#2\@xs@argument@A}%
}

\def\@xs@ldef{\long\def}

\def\@xs@ledef{\long\edef}

% Pas d'expansion des arguments
\def\normalexpandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter{##1}}}
\let\noexpandarg\normalexpandarg% synonyme

% 1-d\'eveloppement du premier token des arguments
\def\expandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

% D\'eveloppement maximum des arguments
\def\fullexpandarg{%
	\let\@xs@def\@xs@ledef% on d\'efinit\@xs@call avec \edef
	\def\@xs@expand##1{##1}% et on neutralise \@xs@expand
}

\def\saveexpandmode{\let\@xs@saved@def\@xs@defarg\let\@xs@saved@expand\@xs@expand}

\def\restoreexpandmode{\let\@xs@defarg\@xs@saved@def\let\@xs@expand\@xs@saved@expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\@xs@ifbeginwithbrace#1{%
	\csname @%
		\expandafter\@gobble\string{%
		\expandafter\@gobble\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@firstoftwo
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\@gobble\string}%
		\@secondoftwo{first}{second}oftwo%
	\endcsname
}

% Cette macro interne prend la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@returnfirstsyntaxunit#1#2{%
	\def\@xs@groupfound{\expandafter\def\expandafter#2\expandafter{\expandafter{#2}}\@xs@gobbleall}% on met #2 dans des accolades et on finit
	\long\def\@xs@assignfirsttok##1##2\@xs@nil{\let\@xs@toks0\def#2{##1}}%
	\def\@xs@testfirsttok{%
		\let\@xs@next\@xs@assignfirsttok
		\ifx\@xs@toks\bgroup
			\expandafter\@xs@ifbeginwithbrace\expandafter{\@xs@argument}{\def\@xs@next{\afterassignment\@xs@groupfound\def#2}}{}%
		\fi
		\@xs@next}%
	\def\@xs@argument{#1}%
	\edef\@xs@next{\expandafter\@xs@beforespace\detokenize{#1} \@xs@nil}% #1 commence par un espace ?
	\ifx\@xs@next\@empty
		\def\@xs@next{\expandafter\ifx\expandafter\@empty\detokenize\expandafter{\@xs@argument}\@empty\let#2\@empty\else\def#2{ }\let\@xs@toks0\fi}%
	\else
		\def\@xs@next{\expandafter\futurelet\expandafter\@xs@toks\expandafter\@xs@testfirsttok\@xs@argument\@xs@nil}%
	\fi
	\@xs@next
}

% Cette macro interne enl\`eve la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@testsecondtoken#1\@xs@nil{\@xs@ifbeginwithbrace{#1}}

\long\def\@xs@gobblespacebeforebrace#1#{}% supprime tout ce qui est avant la 1ere accolade ouvrante

\long\def\@xs@removefirstsyntaxunit#1#2{%
	\def\@xs@argument{#1}%
	\expandafter\expandafter\expandafter\ifx\expandafter\expandafter\expandafter\@empty\expandafter\@xs@beforespace\detokenize\expandafter{\@xs@argument} \@xs@nil\@empty% #1 commence par un espace ?
		\expandafter\@xs@ifempty\expandafter{\@xs@argument}%
			{\let#2\@empty}
			{\afterassignment\@xs@testsecondtoken% après avoir mangé le 1er token, on va tester si la suite commence par «{»
			\expandafter\let\expandafter\@xs@secontoken\expandafter=\expandafter\@sptoken\@xs@argument\@xs@@nil\@xs@nil% on mange le 1er token et on rajoute \@xs@@nil à la fin pour éviter de perdre les accolades du groupe
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@gobblespacebeforebrace\@xs@argument}}%
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@behindspace\@xs@argument\@xs@nil}}%
			}%
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
		\expandafter\expandafter\expandafter{\expandafter\@gobble\@xs@argument}%
	\fi
}

% Macros \`a arguments d\'elimit\'es pour les macros ci dessus
\long\def\@xs@beforespace#1 #2\@xs@nil{#1}

\long\def\@xs@behindspace#1 #2\@xs@nil{#2}

\long\def\@xs@returnfirstsyntaxunit@ii#1#2\@xs@nil{#1}

\long\def\@xs@gobbleall#1\@xs@nil{}

% Cette macro interne est utilis\'ee dans les macros \'etoil\'ees pour :
% 1) d\'evelopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci \`a l'aide de la macro \@xs@def
% 2) Ensuite, on d\'etokenize ce d\'eveloppement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\@xs@expand@and@detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\@xs@expand#1}% on d\'eveloppe #2 selon le mode de d\'eveloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d\'etokenize et on assigne \`a #1
}

\long\def\@xs@expand@and@assign#1#2{\@xs@def#1{#2}}% on d\'eveloppe #2 selon \fullexpandarg ou \normalexpandarg

\long\def\@xs@edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}

\long\def\@xs@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\@xs@argstring{0########1########2########3########4########5########6########7########8########9}

% \@xs@DefArg{3} met dans la sc \@xs@myarg les tokens "####1####2####3"
\def\@xs@DefArg#1{\def\@xs@defarg0##1#1##2\@xs@nil{\def\@xs@myarg{##1#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@DefArg@{3} met dans la sc \@xs@myarg les tokens "[####1]####2####3####4"
\def\@xs@DefArg@#1{\expandafter\@xs@defarg@\expandafter{\number\numexpr#1+1}}

\def\@xs@defarg@#1{\def\@xs@defarg0##11##2#1##3\@xs@nil{\def\@xs@myarg{[##11]##2#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@OneArg{3} met dans la sc \@xs@myarg les tokens "####3"
\def\@xs@OneArg#1{\expandafter\@xs@onearg\expandafter{\number\numexpr#1-1}{#1}}

\def\@xs@onearg#1#2{\def\@xs@defarg##1#1##2#2##3\@xs@nil{\def\@xs@myarg{##2#2}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% #1 : num\'ero du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num\'ero de l'argument devant être d\'etokenis\'e si \'etoile
\def\@xs@BuildLines#1#2#3#4{%
	\let\@xs@newlines\@empty
	\let\@xs@newargs\@empty
	\def\@xs@buildlines##1{%
		\expandafter\@xs@OneArg\expandafter{\number\numexpr##1+#1-1}%
		\edef\@xs@reserved@B{\noexpand\@xs@expand\csname @xs@arg@\romannumeral\numexpr##1\endcsname}%
		\ifnum##1=\@ne% si c'est le premier argument
			\@xs@ifempty{#3}%
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
				\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter[\@xs@reserved@B]}%
				\def\@xs@reserved@B{@xs@def}% ne pas d\'etok\'eniser l'argument optionnel grace au \@xs@def
				}
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
			\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
		\fi
		\edef\@xs@newlines{\unexpanded\expandafter{\@xs@newlines}\expandafter\noexpand\csname\@xs@reserved@B\endcsname\expandafter\noexpand\csname @xs@arg@\romannumeral\numexpr##1\endcsname{\@xs@myarg}}%
		\ifnum##1<#2\relax
			\def\@xs@next{\expandafter\@xs@buildlines\expandafter{\number\numexpr##1+1}}%
			\expandafter\@xs@next
		\fi}%
	\@xs@buildlines\@ne
}

\def\@xs@newmacro{%
	\@ifstar
		{\let\@xs@reserved@D\@empty\@xs@newmacro@}
		{\let\@xs@reserved@D\relax\@xs@newmacro@0}%
}

% #1 : dernier num\'ero de l'argument devant être d\'etokenis\'e
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\@xs@newmacro@#1#2#3#4#5{%
	\edef\@xs@reserved@A{@xs@\expandafter\@gobble\string#2}%
	\edef\@xs@reserved@C{\expandafter\noexpand\csname\@xs@reserved@A @\ifx\@empty#3\@empty @\fi\endcsname}%
	\edef\@xs@reserved@B{%
		\ifx\@empty\@xs@reserved@D
			\def\noexpand#2{\noexpand\@ifstar
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@detokenize\expandafter\noexpand\@xs@reserved@C}%
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
		\fi
		\ifx\@empty#3\@empty
		\else
			\def\expandafter\noexpand\@xs@reserved@C{%
				\noexpand\@testopt{\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname}{\ifx\@xs@def\@xs@ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit :
	% si #3 est vide : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@@}}
	% si #3 existe   : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@}}
	%                  \@xs@NOM@{\@testopt{\@xs@NOM@@}{#3}}}
	\long\@xs@reserved@B
	\ifx\@empty#3\@empty
		\@xs@BuildLines1{#4}{#3}{#1}%
		\@xs@DefArg{#4}%
	\else
		\expandafter\@xs@BuildLines\expandafter1\expandafter{\number\numexpr#4+1}{#3}{#1}%
		\@xs@DefArg@{#4}%
	\fi
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname\@xs@myarg}%
	\edef\@xs@reserved@C{\unexpanded\expandafter{\@xs@newlines}\edef\noexpand\@xs@call}%
	\edef\@xs@reserved@D{%
		\noexpand\noexpand\expandafter\noexpand\csname\@xs@reserved@A\endcsname\unexpanded\expandafter{\@xs@newargs}%
	}%
	\ifnum#5=\@ne\edef\@xs@reserved@D{\noexpand\noexpand\noexpand\@testopt{\unexpanded\expandafter{\@xs@reserved@D}}{}}\fi
	\@xs@edefaddtomacro\@xs@reserved@C{{\unexpanded\expandafter{\@xs@reserved@D}}\noexpand\@xs@call}%
	\@xs@edefaddtomacro\@xs@reserved@B{{\unexpanded\expandafter{\@xs@reserved@C}}}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\@xs@NOM@@[##2]##3##4##5{%
	%          \@xs@def\@xs@arg@i{##2}\@xs@assign\@xs@arg@ii{##3}\@xs@assign\@xs@arg@iii{##4}\@xs@asign\@xs@arg@iv{##5}%
	% si #5=0: \edef\@xs@call{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}%
	% si #5=1: \edef\@xs@call{\noexpand\@testopt{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@i}{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}{}}%
	%          \@xs@call}
	\long\@xs@reserved@B
	\edef\@xs@reserved@B{%
		\def\expandafter\noexpand\csname\@xs@reserved@A\endcsname
			\@xs@myarg\ifnum#5=\@ne[\unexpanded{##}\number\numexpr\ifx\@empty#3\@empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \@xs@NOM[##2]##3##4##5[##6]{#6}
	\long\@xs@reserved@B
}

% macro g\'en\'erique qui lit \@xs@reserved@C us par us
% 3 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atbegingroup      (un groupe vient d'être ouvert)
% \@xs@atnextsyntaxunit  (la future US n'est pas un groupe)
\def\@xs@read@reserved@C{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@read@reserved@C
		\@xs@exploregroups
		\ifx\bgroup\@xs@toks
			\advance\integerpart\@ne
			\begingroup
				\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
				\@xs@manage@groupID
				\let\@xs@nestlevel\@ne
				\integerpart\z@
				\@xs@atbegingroup
		\else
			\global\advance\decimalpart\@ne
			\@xs@atnextsyntaxunit
		\fi
		}%
	\@xs@next
}

% macro g\'en\'erique qui lit \@xs@reserved@D en proc\'edant \`a des tests avec \IfBeginWith
% 2 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atoccurfound      (une occurrence a \'et\'e trouv\'ee)
\def\@xs@read@reserved@D{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}%
		{\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
			{\expandafter\@xs@reserved@D\expandafter}\expandafter{\@xs@reserved@E}%
			{\global\advance\decimalpart\@ne
			\let\@xs@reserved@D\@xs@reserved@A
			\@xs@atoccurfound
			}%
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@A
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
			\let\@xs@next\@xs@read@reserved@D
			\@xs@exploregroups
			\ifx\bgroup\@xs@toks
				\advance\integerpart\@ne
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@D\@xs@reserved@A
					\@xs@manage@groupID
					\let\@xs@reserved@C\@empty
					\let\@xs@nestlevel\@ne
					\integerpart\z@
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro\StrRemoveBraces{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\let\@xs@reserved@B\@empty
	\let\@xs@nestlevel\z@
	\@xs@StrRemoveBraces@i
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#2}%
}

\def\@xs@StrRemoveBraces@i{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@B}%
			\let\@xs@next\@xs@StrRemoveBraces@i
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@StrRemoveBraces@i
		\ifx\bgroup\@xs@toks
			\ifx\@xs@exploregroups\relax% on explore les groupes ?
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
					\let\@xs@nestlevel\@ne
					\integerpart\z@
					\let\@xs@reserved@B\@empty
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\@xs@reserved@A
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
		\fi
		}%
	\@xs@next
}

% \@xs@cutafteroccur coupe l'argument #1 apr\`es la #3\`eme occurrence de #2
% \@xs@reserved@C : contient ce qui se trouve avant cette occurrence
% \@xs@reserved@D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \@xs@reserved@E : contient ce qui se trouve apr\`es l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy\'ees sont vides
\long\def\@xs@cutafteroccur#1#2#3{%
	\ifnum#3<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
		}
		{\@xs@cutafteroccur@i{#1}{#2}{#3}}%
}
	
\long\def\@xs@cutafteroccur@i#1#2#3{%
	\def\@xs@reserved@D{#1}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#2}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\ifnum\decimalpart=\numexpr(#3)\relax % occurrence trouv\'ee ?
		\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\@xs@argument@A}%
	\else
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
	\fi
}

\@xs@newmacro*3\IfSubStr{1}{2}{0}{%
	\def\@xs@argument@A{#2}\def\@xs@argument@B{#3}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur
	\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}{#1}%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*2\IfBeginWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@secondoftwo
		}
		{\def\@xs@next{%
			\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
				{\expandafter\@xs@argument@A\expandafter}\expandafter
				{\@xs@argument@B}}%
		}%
	\@xs@next
}

\long\def\@xs@IfBeginWith@i#1#2{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@firstoftwo% #2 est vide, tous les tests sont pass\'es avec succ\`es : on renvoie #3
		}
		{\expandafter\@xs@ifempty\expandafter{\@xs@argument@A}%
			{\let\@xs@next\@secondoftwo% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
			\ifx\@xs@reserved@A\@xs@reserved@B% il y a \'egalit\'e...
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A% on enl\`eve les 1ere unit\'es syntaxiques
				\def\@xs@next{% et on recommence avec ces arguments racourcis d'1 unit\'e syntaxique
					\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
					\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}}%
			\else
				\let\@xs@next\@secondoftwo
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro*2\IfEndWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\@xs@ifempty{#2}%
		{\let\@xs@reserved@A\@secondoftwo
		}
		{\expandafter\expandafter\expandafter\@xs@StrCount
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter
			{\@xs@argument@B}[\@xs@reserved@A]%
		\ifnum\@xs@reserved@A=\z@
			\let\@xs@reserved@A\@secondoftwo
		\else
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
				{\let\@xs@reserved@A\@firstoftwo}
				{\let\@xs@reserved@A\@secondoftwo}%
		\fi
		}%
	\@xs@reserved@A
}

\@xs@newmacro*4\IfSubStrBefore{1,1}{3}{0}{\@xs@IfSubStrBefore@i[#1]{#2}{#3}{#4}}

\def\@xs@IfSubStrBefore@i[#1,#2]#3#4#5{%
	\def\@xs@reserved@C{#3}%
	\ifx\@xs@exploregroups\relax% si on explore les groupes
		\let\@xs@reserved@B\@empty
		\let\@xs@nestlevel\z@
		\@xs@StrRemoveBraces@i% on retire les accolades
		\let\@xs@reserved@C\@xs@reserved@B
	\fi
	\def\@xs@reserved@A{#5}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#2}%
	\def\@xs@reserved@A{#4}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#1}%
	\global\let\groupID\@empty
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*4\IfSubStrBehind{1,1}{3}{0}{\@xs@IfSubStrBehind@i[#1]{#2}{#3}{#4}}

\long\def\@xs@IfSubStrBehind@i[#1,#2]#3#4#5{\@xs@IfSubStrBefore@i[#2,#1]{#3}{#5}{#4}}

\long\def\@xs@formatnumber#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\@xs@returnfirstsyntaxunit{#1}\@xs@reserved@A
		\def\@xs@reserved@B{+}%
		\ifx\@xs@reserved@A\@xs@reserved@B
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@C
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			 	{\def#2{+0X}}
			 	{\expandafter\def\expandafter#2\expandafter{\expandafter+\expandafter0\@xs@reserved@C}}%
		\else
			\def\@xs@reserved@B{-}%
			\ifx\@xs@reserved@A\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
				\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
					{\def#2{-0X}}%
					{\expandafter\def\expandafter#2\expandafter{\expandafter-\expandafter0\@xs@reserved@A}}%
			\else
				\expandafter\def\expandafter#2\expandafter{\expandafter0\@xs@argument@A}%
			\fi
		\fi
		}%
}

\@xs@newmacro\IfInteger{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\let\@xs@after@intpart\@xs@afterinteger
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\ifnum\decimalpart=\z@
			\let\@xs@next\@firstoftwo% partie décimale constituée de 0 --> seul cas où on renvoie vrai
		\else
			\let\@xs@afterinteger\@xs@after@intpart
			\let\@xs@next\@secondoftwo
		\fi
	\else
		\let\@xs@afterinteger\@xs@after@intpart
		\let\@xs@next\@secondoftwo
	\fi
	\@xs@next
}

\@xs@newmacro\IfDecimal{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}

\long\def\@xs@defafterinteger#1\relax\@xs@nil{\def\@xs@afterinteger{#1}}

\def\@xs@testdot{%
	\let\xs@decsep\@empty
	\@ifnextchar.%
		{\def\xs@decsep{.}\@xs@readdecimalpart}%
		{\@xs@testcomma}%
}

\def\@xs@testcomma{%
	\@ifnextchar,%
		{\def\xs@dessep{,}\@xs@readdecimalpart}%
		{\@xs@endnumber}%
}

\long\def\@xs@readdecimalpart#1#2\@xs@nil{%
	\ifx\@empty#2\@empty
		\def\@xs@reserved@A{0X}%
	\else
		\def\@xs@reserved@A{0#2}%
	\fi
	\afterassignment\@xs@defafterinteger\decimalpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@endnumber\@xs@afterinteger\@xs@nil
}

\long\def\@xs@endnumber#1\@xs@nil{\def\@xs@afterdecimal{#1}}

% test d'\'egalit\'e sur des chaines (et des chaines contenant des nombres)
\long\def\@xs@IfStrEqFalse@i#1#2{\let\@xs@reserved@A\@secondoftwo}
\long\def\@xs@IfStrEqFalse@ii#1#2{% renvoie vrai si les 2 arg sont d\'ecimaux et s'ils sont \'egaux, faux sinon
	\@xs@IfDecimal{#1}%
		{\@xs@IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\@xs@reserved@A\@firstoftwo
			\else
				\let\@xs@reserved@A\@secondoftwo
			\fi% les 2 sont d\'ecimaux : on fait le test
			}%
			{\let\@xs@reserved@A\@secondoftwo}% un seul est d\'ecimal
		}%
		{\let\@xs@reserved@A\@secondoftwo}% #1 n'est pas d\'ecimal
}

\long\def\@xs@TestEqual#1#2{% teste si les 2 arguments sont \'egaux
	\def\@xs@reserved@A{#1}\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\let\@xs@reserved@A\@firstoftwo% \'egalit\'e parfaite des 2 chaines
	\else
		\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}%
	\fi
	\@xs@reserved@A
}

\@xs@newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont \'egales
	\let\@xs@reserved@D\@xs@IfStrEqFalse@i
	\@xs@TestEqual{#1}{#2}%
}

\@xs@newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont \'egaux
	\let\@xs@reserved@D\@xs@IfStrEqFalse@ii
	\@xs@TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfStrEq*}\@xs@IfStrCase}%
		{\def\@xs@reserved@E{\IfStrEq}\@xs@IfStrCase}%
}

\long\def\@xs@IfStrCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\IfEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfEq*}\@xs@IfEqCase}%
		{\def\@xs@reserved@E{\IfEq}\@xs@IfEqCase}%
}

\long\def\@xs@IfEqCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\long\def\@xs@IfStringCase#1#2[#3]{%
	\long\def\@xs@testcase##1##2##3\@xs@nil{% lit les 2 premieres unit\'es syntaxiques dans ##1 et ##2. Les autres dans ##3
		\@xs@reserved@E{#1}{##1}%
			{##2}% le test est positif, on ex\'ecute le code correspondant
			{\@xs@ifempty{##3}%
			 	{#3}% s'il n'y a plus de cas, on ex\'ecute le code <autres cas>
				{\@xs@testcase##3\@xs@nil}% sinon, on recommence avec ce qui reste
			 }%
	}%
	\@xs@testcase#2\@xs@nil
}

% Renvoie ce qui est \`a gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBefore{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
}

% Renvoie ce qui est \`a droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBehind{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\@xs@newmacro*4\StrBetween{1,1}{3}{1}{\@xs@StrBetween@i[#1]{#2}{#3}{#4}[#5]}

\long\def\@xs@StrBetween@i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\@xs@cutafteroccur{#3}{#5}{#2}%
		\expandafter\@xs@cutafteroccur\expandafter{\@xs@reserved@C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#6}%
	\global\let\groupID\@empty
}

\def\exploregroups{\let\@xs@exploregroups\relax}

\def\noexploregroups{\def\@xs@exploregroups{\let\@xs@toks0\relax}}

\def\saveexploremode{\let\@xs@saveexploremode\@xs@exploregroups}

\def\restoreexploremode{\let\@xs@exploregroups\@xs@saveexploremode}

% Remplace les #1 premi\`eres occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\@xs@newmacro\StrSubstitute{0}{3}{1}{%
	\def\@xs@reserved@D{#2}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#3}%
	\def\@xs@argument@C{#3}\def\@xs@argument@D{#4}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum#1<\@ne
			\let\@xs@reserved@A\@xs@argument@D
		\else
			\ifnum\decimalpart>#1
				\let\@xs@reserved@A\@xs@argument@C
			\else
				\let\@xs@reserved@A\@xs@argument@D
			\fi
		\fi
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		\@xs@read@reserved@D
	}%
	\@xs@ifempty{#3}%
		{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#5}%
		}
		{\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#5}%
		}%
}

% Supprime les #1 premi\`eres occurrences de #3 dans #2
\@xs@newmacro\StrDel{0}{2}{1}{\@xs@StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\@xs@exitallgroups{\ifnum\@xs@nestlevel>\z@\endgroup\expandafter\@xs@exitallgroups\fi}

% Compte combien d'unit\'es syntaxiques contient la chaine #1 ?
\@xs@newmacro\StrLen{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\decimalpart\z@
	\let\@xs@nestlevel\z@
	\gdef\groupID{0}%
	\let\@xs@atbegingroup\relax
	\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
	\let\@xs@atnextsyntaxunit\relax
	\@xs@read@reserved@C
	\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n\'ecessaire pour trouver une unit\'e syntaxique derri\`ere
\def\@xs@continuetonext{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel>\z@
			\expandafter\endgroup\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}% on concat\`ene
			\expandafter\expandafter\expandafter\@xs@continuetonext% on recommence
		\fi}
		\relax
}%

\def\@xs@manage@groupID{%
	\begingroup\def\@xs@reserved@A{0}%
	\ifx\@xs@reserved@A\groupID% si on arrive du groupe de niveau 0
		\endgroup
		\xdef\groupID{\number\integerpart}% on met simplement le niveau
	\else
		\endgroup
		\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\groupID\expandafter\expandafter\expandafter{\expandafter\groupID\expandafter,\number\integerpart}%
	\fi
}

% Cette macro coupe la chaine #1 apr\`es l'unit\'e syntaxique n°#2
\def\StrSplit{%
	\@ifstar
		{\let\@xs@reserved@E\@xs@continuetonext\StrSpl@t}%
		{\let\@xs@reserved@E\relax\StrSpl@t}%
}

\@xs@newmacro\StrSpl@t{}{2}{0}{\@xs@StrSplit@i{#2}{#1}\@xs@StrSplit@ii}

% Cette macro interne coupe la chaine #2 apr\`es l'unit\'e syntaxique n°#1
% Le d\'ebut est assign\'e dans \@xs@reserved@B et la fin dans \@xs@reserved@C
\long\def\@xs@StrSplit@i#1#2{%
	\def\@xs@reserved@D{#1}%
	\def\@xs@reserved@C{#2}%
	\let\@xs@reserved@B\@empty
	\global\let\groupID\@empty
	\ifnum#1>\z@
		\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
			\@xs@read@reserved@C
		}%
		\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
		\def\@xs@atnextsyntaxunit{%
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
			\ifnum\decimalpart=\@xs@reserved@D\relax
				\ifx\@xs@reserved@C\@empty\@xs@reserved@E\fi
				\global\let\@xs@reserved@B\@xs@reserved@B
				\global\let\@xs@reserved@C\@xs@reserved@C
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
}

\def\@xs@StrSplit@ii#1#2{\let#1\@xs@reserved@B\let#2\@xs@reserved@C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\@xs@newmacro*3\StrCut{1}{2}{0}{%
	\@xs@ifempty{#3}%
		{\global\let\groupID\@empty
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		}
		{\ifnum#1<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\@xs@StrCut@ii{#2}{#3}1}
			{\@xs@StrCut@ii{#2}{#3}{#1}}%
		}%
	\@xs@StrCut@iii
}

\long\def\@xs@StrCut@ii#1#2#3{%
	\def\@xs@reserved@D{#1}%
	\let\@xs@reserved@C\@empty
	\def\@xs@reserved@E{#2}%
	\decimalpart\z@\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi
	}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter
	\def
		\expandafter\expandafter\expandafter
	\@xs@reserved@D
		\expandafter\expandafter\expandafter
	{\expandafter\@xs@reserved@C\@xs@argument@A}%
}

\long\def\@xs@StrCut@iii#1#2{\let#1\@xs@reserved@C\let#2\@xs@reserved@E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit\'es syntaxiques aux positions compris !
\@xs@newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\@xs@reserved@E\relax
		\@xs@StrSplit@i{#3}{#1}%
		\edef\@xs@reserved@C{\number\numexpr#2-1}%
		\let\@xs@reserved@E\relax
		\expandafter\expandafter\expandafter\@xs@StrSplit@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@B}%
	\expandafter\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
	\global\let\groupID\@empty
}

% supprime #2 unit\'es syntaxiques \`a gauche dans la chaine #1
\@xs@newmacro\StrGobbleLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

% extrait de #1 la chaine \`a gauche de longueur #2
\@xs@newmacro\StrLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% supprime #2 unit\'es syntaxiques \`a droite dans la chaine #1
\@xs@newmacro\StrGobbleRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% renvoie #2 unit\'es syntaxiques \`a la droite de la chaine #1
\@xs@newmacro\StrRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

\@xs@newmacro\StrChar{}{2}{1}{%
	\let\@xs@reserved@B\@empty
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\ifnum#2>\z@
		\def\groupID{0}\let\@xs@nestlevel\z@\integerpart\z@\decimalpart\z@
		\let\@xs@atbegingroup\relax
		\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
		\def\@xs@atnextsyntaxunit{%
			\ifnum\decimalpart=\@xs@reserved@D% la n i\`eme US est atteinte ?
				\global\let\@xs@reserved@B\@xs@reserved@A% on capture l'US en cours qui est celle cherch\'ee
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@B}%
		{\global\let\groupID\@empty}
		\relax
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\@xs@newmacro\StrCount{}{2}{1}{%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@E{#2}\let\@xs@reserved@C\@empty
	\@xs@ifempty{#2}%
		{\@xs@ReturnResult{0}{#3}}
		{\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
			\@xs@read@reserved@D
		}%
		\def\@xs@atoccurfound{\let\@xs@reserved@C\@empty\@xs@read@reserved@D}%
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro\StrPosition{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\let\@xs@reserved@E\groupID
	\ifx\@xs@reserved@C\@xs@reserved@D
		\@xs@ReturnResult{0}{#4}%
		\let\@xs@reserved@E\@empty
	\else
		\expandafter\@xs@StrLen\expandafter{\@xs@reserved@C}[\@xs@reserved@C]%
		\expandafter\@xs@ReturnResult\expandafter{\number\numexpr\@xs@reserved@C+1}{#4}%
	\fi
	\global\let\groupID\@xs@reserved@E
}

\def\comparestrict{\let\@xs@comparecoeff\@ne}

\def\comparenormal{\let\@xs@comparecoeff\z@}

\def\savecomparemode{\let\@xs@saved@comparecoeff\@xs@comparecoeff}

\def\restorecomparemode{\let\@xs@comparecoeff\@xs@saved@comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont \'egaux et renvoie la
% position de la premiere unit\'e syntaxiques diff\'erente sinon
\@xs@newmacro*2\StrCompare{}{2}{1}{%
	\def\@xs@reserved@A{#1}%
	\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@B\@xs@reserved@A
		\@xs@ReturnResult{0}{#3}%
	\else
		\def\@xs@next{\@xs@StrCompare@i{#1}{#2}{#3}}%
		\expandafter\@xs@next
	\fi
}

\long\def\@xs@StrCompare@i#1#2#3{%
	\def\@xs@StrCompare@iii##1{%
		\let\@xs@reserved@A\@empty
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@reserved@A{*\@xs@comparecoeff}}%
			{\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
				{\def\@xs@reserved@A{*\@xs@comparecoeff}}
				\relax
			}%
		\def\@xs@next{%
			\expandafter\@xs@ReturnResult\expandafter
			{\number\numexpr##1\@xs@reserved@A\relax}{#3}%
		}%
	}%
	\def\@xs@StrCompare@ii##1{% ##1 est la position
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@B
		\ifx\@xs@reserved@B\@xs@reserved@A
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
				{\@xs@StrCompare@iii{##1}% les 2 unit\'es syntaxiques sont \'egales, on renvoie la position
				}
				{\def\@xs@next{\expandafter\@xs@StrCompare@ii\expandafter{\number\numexpr##1+1}}% les 2 unit\'es syntaxiques sont \'egales et non vides, on recommence
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
				}%
		\else% les 2 unit\'es syntaxiques sont diff\'erentes : on renvoie la position
			\@xs@StrCompare@iii{##1}%
		\fi
		\@xs@next
	}%
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\@xs@StrCompare@ii1%
}

\@xs@newmacro\StrFindGroup{}{2}{1}{%
	\def\@xs@reserved@A{#2}\def\@xs@reserved@B{0}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\def\@xs@next{\@xs@ReturnResult{{#1}}{#3}}%
	\else
		\def\@xs@next{\@xs@StrFindGroup@i{#1}{#2}[#3]}%
	\fi
	\@xs@next
}

\long\def\@xs@StrFindGroup@i#1#2[#3]{%
	\def\@xs@StrFindGroup@ii{%
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@next{\@xs@ReturnResult{}{#3}}% s'il ne reste plus rien, on renvoie vide
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@D
			\ifx\bgroup\@xs@toks% si la 1\`ere unit\'e syntaxique est un groupe explicite
				\advance\decimalpart\@ne% on augmente le compteur
				\ifnum\decimalpart=\@xs@reserved@A% on est au groupe cherch\'e lors de la profondeur courante ?
					\ifx\@empty\@xs@reserved@B% on est \`a la profondeur maximale ?
						\def\@xs@next{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#3}}% on renvoie ce groupe
					\else% sinon
						\expandafter\def\expandafter\@xs@next\expandafter{\expandafter\@xs@StrFindGroup@i\@xs@reserved@D}% on recommence avec ce groupe
						\expandafter\@xs@addtomacro\expandafter\@xs@next\expandafter{\expandafter{\@xs@reserved@B}[#3]}% et les profondeurs de recherche restantes
					\fi
				\else
					\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
					\let\@xs@next\@xs@StrFindGroup@ii
				\fi
			\else
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\let\@xs@next\@xs@StrFindGroup@ii
			\fi
			}%
		\@xs@next
	}%
	\@xs@extractgroupnumber{#2}\@xs@reserved@A\@xs@reserved@B
	\decimalpart\z@
	\ifnum\@xs@reserved@A>\z@\def\@xs@reserved@C{#1}\else\let\@xs@reserved@C\@empty\fi
	\@xs@StrFindGroup@ii
}

\def\@xs@extractgroupnumber#1#2#3{%
	\def\@xs@extractgroupnumber@i##1,##2\@xs@nil{\def#2{##1}\def#3{##2}}%
	\@xs@extractgroupnumber@i#1,\@xs@nil
	\ifx\@empty#3\else\@xs@extractgroupnumber@i#1\@xs@nil\fi
}

\def\expandingroups{\let\@xs@expandingroups\exploregroups}

\def\noexpandingroups{\let\@xs@expandingroups\noexploregroups}

\def\StrExpand{\@testopt{\@xs@StrExpand}{1}}
\long\def\@xs@StrExpand[#1]#2#3{%
	\begingroup
		\@xs@expandingroups
		\ifnum#1>\z@
			\integerpart#1\relax
			\decimalpart\z@
			\gdef\groupID{0}%
			\let\@xs@nestlevel\z@
			\def\@xs@atendofgroup{%
				\expandafter\endgroup
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
				\@xs@read@reserved@C
			}%
			\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
			\def\@xs@atnextsyntaxunit{%
				\expandafter\expandafter\expandafter\@xs@addtomacro
				\expandafter\expandafter\expandafter\@xs@reserved@B
				\expandafter\expandafter\expandafter{\@xs@reserved@A}%
			}%
			\def\@xs@reserved@C{#2}%
			\@xs@StrExpand@i{#1}% Appel de la macro r\'ecursive
		\else
			\def\@xs@reserved@B{#2}%
		\fi
		\global\let\@xs@reserved@B\@xs@reserved@B
	\endgroup
	\let#3\@xs@reserved@B
	\global\let\groupID\@empty
}

\long\def\@xs@StrExpand@i#1{%
	\ifnum#1>\z@
		\let\@xs@reserved@B\@empty
		\@xs@read@reserved@C
		\let\@xs@reserved@C\@xs@reserved@B
		\def\@xs@reserved@A{\expandafter\@xs@StrExpand@i\expandafter{\number\numexpr#1-1}}%
	\else
		\let\@xs@reserved@A\relax
	\fi
	\@xs@reserved@A
}

\def\scancs{\@testopt{\@xs@scancs}{1}}
\long\def\@xs@scancs[#1]#2#3{%
	\@xs@StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

% Restaure le code de @
\catcode`\@=\CurrentAtCatcode\relax

% D\'efinit le d\'elimiteur verb
% d\'efinit les diff\'erents modes et les m\'emorise
\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput
%
% Historique
%------------------------------------------------------------------------------
%% v1.0    4/7/2008 : - Package achev\'e.
%          7/7/2008 : - Package publi\'e sur CTAN.
%------------------------------------------------------------------------------
% v1.1    15/8/2008
%   - Le package ne n\'ecessite plus LaTeX et est d\'esormais utilisable sous
%     Plain eTeX.
%   - Ajout des macros \IfInteger et \IfDecimal.
%     Pour cette derni\`ere, la partie enti\`ere et la partie d\'ecimale sont
%     r\'ecup\'erables dans les compteurs \integerpart et \decimalpart. Ce
%     qu'il reste apr\`es qu'un caract\`ere non attendu soit rencontr\'e est
%     dispo dans \@xs@remainafterdecimal
%   - Correction d'un bug dans \tokenize :
%        suppression de l'expansion avec \normalexpandarg pour \'eviter le bug
%        avec les lettres accentu\'ees dans l'exemple : \tokenize\aa{\'e\`u}
%   - Am\'elioration du code de la plupart des macros.
%   - \'Ecriture d'une routine \@xs@newmacro d\'efinissant les  macros.
%   - Suppression de tous les compteurs grace \`a \numexpr.
%   - Nouvelles fonctionnalit\'es internes dans :
%      \IfSubStr
%        ajout des chaines se trouvant avant et apr\`es l'occurrence test\'ee
%        dans les sc \@xs@behind@IfSubStr et \@xs@before@IfSubStr
%      \StrCount
%        a) ajout de ce qui se trouve apr\`es la derni\`ere occurrence dans la
%           sc \@xs@StrCount@afterlastocccur
%        b) la macro ne d\'epend plus d'aucune autre
%------------------------------------------------------------------------------
% v1.2    23/8/2008
%   - Am\'elioration du code de \StrMid \StrGobbleLeft, \StrLeft,
%     \StrGobbleRight et \StrRight \`a l'aide de la nouvelle macro
%     \@xs@StrSplit@i
%   - Nouveau test \IfStrEq qui compare 2 chaines
%   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
%     contiennent un nombre)
%   - Correction d'un bug dans \@xs@formatnumber. La macro n'envisageait pas le
%     cas o\`u son argument \'etait vide ce qui faiasait planter
%     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
%------------------------------------------------------------------------------
% v1.3    21/9/2008
%  - Am\'elioration du code, mise en place de r\'ecursivit\'es terminales dans
%    toutes les macros r\'ecursives, simplification de \@xs@TestEqual en
%    utilisant \ifx
%  - Nouvelles macros \IfStrEqCase et \IfEqCase
%      Teste si une chaîne est \'egale \`a plusieurs cha\^ines donn\'ee et
%      ex\'ecute un code sp\'ecifique
%  - Cr\'eation de la macro publique \StrSplit
%      Coupe la chaine en 2 \`a une position donn\'ee
%  - Nouvelle macro \StrCompare
%      Compare 2 chaînes et renvoie la position du 1er caract\`ere diff\'erent.
%      Renvoie 0 si elles sont \'egales.
%------------------------------------------------------------------------------
% v1.3a   29/9/2008
%  - Correction d'un bug : \expandafter#1
%    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
%    nombre > 9 !
%  - R\'e \'ecriture de \@xs@returnfirstsyntaxunit et \@gobble qui
%    deviennent purement d\'eveloppables.
%  - R\'e \'ecriture de \StrLen
%  - Nouvelle macro interne \@xs@cutafteroccur
%      Coupe la chaine apr\`es la ni\`eme occurrence d'une sous chaine.
%  - Code am\'elior\'e de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
%    \StrGobbleRight grace \`a \@xs@cutafteroccur
%------------------------------------------------------------------------------
% v1.4   4/11/2008
%  - xstring traite ses arguments par unit\'e syntaxique, et donc toutes les
%    macros internes ont \'et\'e r\'e-\'ecrites \`a cette fin.
%  - Le manuel a \'et\'e r\'e-\'ecrit, rendu plus clair et mieux structur\'e.
%  - Nouvelle fonctionnalit\'e : \expandarg
%      le 1er lex\`eme de chaque argument est 1-d\'evelopp\'e avant que la
%      macro ne soit appel\'ee. Si un argument comporte plus qu'1 lex\`eme,
%      il faut passer par \scancs*[1] pour 1-d\'evelopper toutes les unit\'es
%      syntaxiques.
%  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
%    d\'efaut dans \StrSubstitute et \StrDel
%  - Coh\'erence dans les nom des s\'equences de contr\^oles temporaires qui
%    sont d\'esormais : \@xs@reserved@A \`a \@xs@reserved@E
%------------------------------------------------------------------------------
% v1.4a  12/11/2008
%  - Correction d'un bug dans \@xs@StrSplit dans le cas o\`u l'argument
%     num\'erique est <1 : la 1ere coupure doit être vide et le seconde doit
%     être \'egale \`a l'argument.
%------------------------------------------------------------------------------
% v1.4b  16/11/2008
%  - Correction de 2 bugs dans \@xs@returnfirstsyntaxunit
%------------------------------------------------------------------------------
% v1.5   31/12/2008
%  - Nouvelles fonctionnalit\'es dans la recherche de groupes par un
%    identificateur caract\'erisant leur imbrication. Impl\'ementation de :
%      1) \StrFindGroup
%      2) \groupID
%  - Ajout des nouvelles macros g\'en\'eriques \@xs@read@reserved@C et
%    \@xs@read@reserved@D
%  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
%    que \truc contenait «a{a}».
%  - Correction d'un bug dans \@xs@newmacro : l'argument optionnel \'etait
%    d\'etok\'enis\'e \`a tort dans les macros \'etoil\'ees.
%  - Dans \@xs@newmacro, on doit choisir le num\'ero du dernier argument devant
%    être d\'etok\'enis\'e dans le cas d'une macro \'etoil\'ee (sachant que
%     l'argument optionnel ne l'est jamais)
%------------------------------------------------------------------------------
% v1.5a  09/2/2009
%  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
%    indépendante du mode d'exploration et dispose de ses propres commandes
%    d'exploration : \expandingroups et \noexpandingroups
%  - R\'e-\'ecriture de \scancs, qui devient triviale puisque d\'ependant de
%    \StrExpand. Il n'y a plus de version \'étoil\'ee et d\'esormais, \scancs
%    est sensible au mode d'exploration.
%  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
%  - Correction de bugs : mettre \let\@xs@reserved@E\relax avant d'appeler
%    \@xs@StrSplit@i
%  - Suppression des messages d'erreur, de warning et d'info. xstring devient
%    donc silencieux ;)
%  - Passage de 3 \'a 2 compteurs
%  - Le manuel est d\'esormais plus color\'e, en esp\'erant qu'il sera un peu
%    plus agr\'eable \`a lire !
%------------------------------------------------------------------------------
% v1.5b  13/3/2009
%  - Modification d'un grand nombre de macros de telle sorte que vraiment
%    n'importe quel code peut d\'esormais \^etre plac\'e dans les arguments des
%    macros (comme par exemple des \if, \ifx ou autre, m\^eme sans leur \fi, ce
%    qui n'\'etait pas possible jusqu'alors)
%------------------------------------------------------------------------------
% v1.5c  05/6/2009
%  - Correction d'un bug dans \IfBeginWith : il faut appeler
%    \@xs@returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
%    non pas l'inverse pour que \@xs@toks reflète ce qui se trouve dans #1
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit au cas où #1 commence
%    par un espace : mettre \@xs@toks à 0
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit :
%    \@xs@returnfirstsyntaxunit{{}}\truc
%    faisait que \truc se développait en un espace.
%  - Correction d'un bug dans \@xs@removefirstsyntaxunit où le cas
%    \@xs@removefirstsyntaxunit{ {b}}\truc
%    donnait \truc se développant en «b» au lieu de «{b}».
%------------------------------------------------------------------------------
% v1.5d  28/3/2010
%  - Correction d'un bug dans \IfInteger : \@xs@afterinteger ne donnait pas le
%    bon r\'esultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
%  - \xs@formatnumber ne detokenize plus ses arguments (que m'est-il pass\'e
%    par la t\^ete pour que je code un truc comme ca ?), et donc
%    \@xs@afterinteger et \@xs@afterdecimal ont des tokens ayant le bon
%    catcode
%------------------------------------------------------------------------------
% v1.6  24/10/2012
%  - Correction d'un bug dans \@xs@cutafteroccur au cas o\`u #3<1
%  - \IfDecimal ne \detokenize plus l'argument.
%  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
%    \'etait entre accolades
%  - Nouvelle macro \StrCut
%  - \@xs@cutafteroccur@i ne produit plus d'espace indésirable si #3 était
%    évalué par \numexpr
%------------------------------------------------------------------------------
% v1.7  13/1/2013
%  - Correction d'un manque de rigueur dans les assignations concernant
%    \groupID : elles sont toutes globales d\'esormais
%  - Les macros de xstring sont \long
%------------------------------------------------------------------------------
% v1.7a 28/2/2013
%  - Correction d'un espace parasite dans \@xs@removefirstsyntaxunit
%------------------------------------------------------------------------------
% v1.7b 29/7/2013
%  - La date contenue dans \xstringdate est désormais conforme
%------------------------------------------------------------------------------
% v1.7c 13/10/2013 
%  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
